Winemaking: Extracting Essential Insights for Efficient Threat Detection in Audit Logs

Advanced Persistent Threats (APTs) are continuously evolving, leveraging their stealthiness and persistence to put increasing pressure on current provenance-based Intrusion Detection Systems (IDS). This evolution exposes several critical issues: (1) The dense interaction between malicious and benign nodes within provenance graphs introduces neighbor noise, hindering effective detection; (2) The complex prediction mechanisms of existing APTs detection models lead to the insufficient utilization of prior knowledge embedded in the data; (3) The high computational cost makes detection impractical. To address these challenges, we propose Winemaking, a lightweight threat detection system built on a knowledge distillation framework, capable of node-level detection within audit log provenance graphs. Specifically, Winemaking applies graph Laplacian regularization to reduce neighbor noise, obtaining smoothed and denoised graph signals. Subsequently, Winemaking employs a teacher model based on GNNs to extract knowledge, which is then distilled into a lightweight student model. The student model is designed as a trainable combination of a feature transformation module and a personalized PageRank random walk label propagation module, with the former capturing feature knowledge and the latter learning label and structural knowledge. After distillation, the student model benefits from the knowledge of the teacher model to perform precise threat detection. We evaluate Winemaking through extensive experiments on three public datasets and compare its performance against several state-of-the-art IDS solutions. The results demonstrate that Winemaking achieves outstanding detection accuracy across all scenarios and the detection time is 1.4 to 5.2 times faster than the current state-of-the-art methods.

==> definition.tex <==
\section{Threat Model}
\label{sec:definition}

To build a more comprehensive threat model, we assume certain attacker behaviors and their interactions with system performance. We consider Advanced Persistent Threat (APTs) attackers, who aim to infiltrate a target host through network channels, pre-installed backdoors, or software vulnerabilities. This process is often highly stealthy and can persist for an extended period. During the intrusion, attackers attempt to blend their malicious activities with legitimate background data to obscure their intent. For instance, they may use *Living-off-the-land* techniques, injecting malicious code into legitimate processes, which then spawn new legitimate processes to continue their malicious actions. 

Although the attackers' behavior is highly covert, audit logs capture complete, traceable evidence and footprints of their activities. As in most of the existing works in this field【】, we assume that the underlying operating system, audit framework, and system hardware are intact and trustworthy. Additionally, we assume that attackers cannot directly tamper with the contents of the audit logs, ensuring that the provenance graph constructed by Vodka remains reliable.

==> motivation.tex <==
\section{Attack scenes}
\label{sec:scene}

%\begin{figure*}
%    \centering
%    \includegraphics[width=0.98\textwidth]{figs/mov8_28_3.png}
%    \vspace{-0.1in}
%    \caption{These four summarized diagrams are sourced from the DARPA dataset and depict various network attack activities. In these diagrams, Rectangles, ovals, and diamonds represent processes, files, and sockets, respectively. Black nodes represent benign entities, while red nodes indicate malicious entities.}
%    \Description{A figure illustrating four scenes.}
%    \label{fig:motivation}
%    \vspace{-0.1in}
%\end{figure*}

\subsection{Motivating Example}
This is an attack case from the DARPA E3 CADETS dataset, where the attacker establishes a connection with the Nginx server via IP address 81.49.200.166 and gains shell access. Using the shell, the attacker downloads a malicious payload to /tmp/vUgefal and executes it. The process vUgefal then moves laterally to 61.167.39.128, completes the infection, and further injects sshd into the system, downloading another payload to /var/log/devc. Figure [ ] illustrates our motivating example, where three types of nodes represent system entities, and the lines indicate the directional interactions between them.

\subsection{Limitations to Existing Solutions}
Learning-based detection methods are currently the most promising in the field of threat detection. Their core principle is to build anomaly models by learning from large datasets and then infer whether anomalous behavior represents a malicious attack. Some of the most notable recent works include:
\textbf{MAGIC}, which performs efficient detection by masking the graph and reducing costs;
\textbf{KAIROS}, which identifies four dimensions of intrusion detection systems and uses an encoder-decoder architecture to detect attacks and reconstruct attack chains;
\textbf{THREATRACE}, the first detector to propose behavior pattern construction for each type of node in the provenance graph to achieve node-level detection;
\textbf{ShadeWatcher}, which introduces recommendation system techniques into provenance graph detection and achieves edge-level detection;
\textbf{Unicorn}, which builds a provenance graph enriched with semantics and historical information to capture long-term stealthy attacks.
Although these works demonstrate excellent performance in threat detection, they still face limitations when tested in real-world environments. These limitations are what Vodka aims to address, as shown in Table [ ].

\begin{itemize}[leftmargin=*]
\item \textbf{Neighbor Denoising}:
Provenance graphs constructed from audit logs contain rich information, with nodes and edges representing different meanings. However, current approaches seem too eager to move directly to graph representation learning without adequately addressing the noise in the initial graph. We observed that only Magic acknowledged this issue.

\item \textbf{Lightweight Models}:
One of the major challenges of current log provenance algorithms lies in the large and difficult-to-deploy models. Most existing works use GNN models that, while achieving good performance due to their multi-layer architectures and extensive parameter inputs, make the entire model bloated.

\item \textbf{Low-Cost Detection}:
High memory and time costs during detection render many detectors impractical for real-world deployment. We note that, similarly, only Magic has optimized for performance costs.

\item \textbf{Attack Reconstruction}:
A simple and complete attack chain helps security analysts better understand the attack behavior. However, from a large number of anomalous nodes detected at the node level, we need to reconstruct these attack paths based on the dependency relationships between kernel objects, as exemplified by KAIROS, to enable analysts to respond quickly.

\item \textbf{Granularity}:
Different detection granularities yield different levels of attack discovery. For example, graph-level granularity, as in Unicorn, is easy to partition but lacks the precision to pinpoint specific malicious entities in the graph. Edge-level granularity, as in ShadeWatcher, offers more detailed insights into specific edge relationships but incurs higher detection costs, as the number of edges in a provenance graph is far greater than the number of nodes. Detection methods like Magic, KAIROS, and THREATRACE, which utilize node-level granularity, can target specific entities without requiring detailed learning of edge relationships.

\end{itemize}
